Scaling Laws for Data Filtering -- Data Curation cannot be Compute Agnostic

Vision-language models (VLMs) are trained for thousands of GPU hours on carefully curated web datasets. In recent times, data curation has gained prominence with several works developing strategies to retain 'high-quality' subsets of 'raw' scraped data. For instance, the LAION public dataset retained only 10% of the total crawled data. However, these strategies are typically developed agnostic of the available compute for training. In this paper, we first demonstrate that making filtering decisions independent of training compute is often suboptimal: the limited high-quality data rapidly loses its utility when repeated, eventually requiring the inclusion of 'unseen' but 'lower-quality' data. To address this quality-quantity tradeoff ($\texttt{QQT}$), we introduce neural scaling laws that account for the non-homogeneous nature of web data, an angle ignored in existing literature. Our scaling laws (i) characterize the $\textit{differing}$ 'utility' of various quality subsets of web data; (ii) account for how utility diminishes for a data point at its 'nth' repetition; and (iii) formulate the mutual interaction of various data pools when combined, enabling the estimation of model performance on a combination of multiple data pools without ever jointly training on them. Our key message is that data curation $\textit{cannot}$ be agnostic of the total compute that a model will be trained for. Our scaling laws allow us to curate the best possible pool for achieving top performance on Datacomp at various compute budgets, carving out a pareto-frontier for data curation. Code is available at https://github.com/locuslab/scaling_laws_data_filtering.

==> main_fig.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
    \centering
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/FADU-repeated.pdf}
        \label{fig:task}
    \end{minipage}%
    ~ %
    \begin{minipage}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/pareto_clip.pdf}
        \label{fig:pareto_clip}
    \end{minipage}%
    \vspace{-10pt}
    \label{fig:title_figure}
    \captionof{figure}{\textbf{(a)} \textbf{The Dynamic Problem of Data Filtering}: Web data is non-homogenous, and past work has succeeded at ranking various data subsets according to their diminishing quality (y-axis). However, training on `high-quality' data for multiple epochs leads to diminishing utility (x-axis), an angle ignored in past work. Assume we have both data and compute equivalent to 6 data pools, one could train on the best pool (E) for 6 epochs, or train on the best two pools (E and D) for 2 epochs each, or train on the best 3 pools for 2 epochs each, and so on. Our work aims to answer---\textit{what is the best allocation of, and return for computational resources?} \textbf{(b)} \textbf{Pareto Filtering:} While retaining top-30\% data, based on CLIP score is a widely used data filtering approach for vision-language model training, we show that depending on the ratio of compute to data pool size, we must adaptively make the filtering less (or more) aggressive to account for the diminishing utility of good data with repetitions. The models are trained on a global data pool size of 128M image-caption pairs, and varying compute scales.}
    \vspace{18pt}
}]
